Comparing Large Language Models and Traditional Machine Translation Tools for Translating Medical Consultation Summaries: A Pilot Study

This study evaluates how well large language models (LLMs) and traditional machine translation (MT) tools translate medical consultation summaries from English into Arabic, Chinese, and Vietnamese. It assesses both patient, friendly and clinician, focused texts using standard automated metrics. Results showed that traditional MT tools generally performed better, especially for complex texts, while LLMs showed promise, particularly in Vietnamese and Chinese, when translating simpler summaries. Arabic translations improved with complexity due to the language's morphology. Overall, while LLMs offer contextual flexibility, they remain inconsistent, and current evaluation metrics fail to capture clinical relevance. The study highlights the need for domain-specific training, improved evaluation methods, and human oversight in medical translation.

==> sections/exp.tex <==
\section{Statistical Analysis}
\input{figs/metricTable}
We chose a wide variety of statistical metrics used in Machine Translation domain to obtain an as comprehensive as possible aspect for each generated summary.
These were BLEU, CHR-F and METEOR.
A brief description of each metric and their limitations are listed in Table \ref{tab:metric}. 
The values of each metric range from 0 to 1, where 1 indicates an identical matching between reference translation and generated translation,
while 0 indicates no overlapping at all.

BLEU measures the surface similarity at the word level compared to the reference translation. 
A high score in BLEU means medical terminology, symptoms or diagnoses are captured accurately.
CHR-F measures the surface similarity at the character level compared to the reference translation, which handles morphological variation better in Arabic and Vietnamese.
A high CHR-F score means the generated translation is capturing medical jargon especially abbreviations better. 
METEOR measures similarity in semantic level. A high METEOR score makes sure that even if a medical condition or advice is expressed differently, the core semantic content is still preserved.
%COMET is a machine-generated score that intends to capture overall meaning, fluency and adequacy altogether.
%A high COMET score shows that the machine-generated summary effectively captures the overall meaning, fluency, and adequacy of the consultation, including the patient’s concerns, the doctor’s advice, and the recommended treatment plan.



%\footnote{May need a human sanity check, LLAMA is missing medicine, making up medicine, manual work to line up the translations. penalty for using dot or number or star for bullet point, also penalty for formatting}

==> sections/introduction_backup.tex <==
\section{Introduction}

Machine translation (MT) has witnessed significant advancements with the emergence of large language models (LLMs), revolutionizing the landscape of automatic translation. Traditionally, neural machine translation systems, such as Google Translate, DeepL, and Bing MS Translate, have dominated the field by leveraging sequence-to-sequence models. However, recent developments in LLMs, such as GPT-4, GEMMA-2-27B, and LLAMA-3.1-405B, have raised questions about whether LLM-based approaches can outperform traditional MT systems, particularly in domain-specific translations such as medical texts.

LLMs have demonstrated remarkable proficiency in document-level machine translation by preserving coherence, discourse structure, and contextual consistency~\cite{LLM_translation_quality}. Unlike traditional phrase-based or sequence-based models, LLMs utilize large-scale contextual embeddings, allowing them to handle complex linguistic structures and ensure semantic fidelity across lengthy texts. This is particularly valuable in medical translation, where maintaining precise terminology and accurate medical inferences is of utmost importance~\cite{noll2023machine}.

Despite their zero-shot learning capabilities, LLMs face several challenges when applied to translation. Issues such as idiomatic expressions, terminological consistency, and domain-specific precision remain significant hurdles~\cite{donthi2024improving}. Moreover, effective prompt engineering is crucial to optimizing LLM-based translation, as shown in recent research on optimized prompt techniques~\cite{zhang2023prompting}. Although few-shot learning strategies have improved translation quality~\cite{garcia2023unreasonable}, it remains unclear whether LLMs can consistently outperform dedicated MT models in specialized domains.

\subsection{Medical Machine Translation: Challenges and Considerations}

Medical translation presents a unique challenge due to its technical terminology, critical accuracy requirements, and context-dependent nuances. Errors in medical translation can have severe consequences for patient safety, which requires precision, consistency, and clarity~\cite{costa2012machine, duvsek2014machine}. Traditional statistical and rule-based MT methods have struggled to handle medical terminology effectively, leading to the development of controlled languages to mitigate ambiguities, particularly in translating English-to-Chinese medical protocols~\cite{cardey2004designing}.

Recent advances in LLM-based medical translation suggest that fine-tuning with human evaluation data can significantly improve translation accuracy and fluency~\cite{elshin2024general}. Furthermore, research on multilingual LLMs
challenges the notion that English should remain the central language for multilingual MT, with findings suggesting that alternative linguistic structures could enhance multilingual performance~\cite{diandaru2024linguistic}. 
%Furthermore, the use of minimum Bayes risk decoding and LLM reranking has been shown to improve document-level translation consistency~\cite{kudo2024document}.

\subsection{LLMs in Translation Evaluation and Quality Estimation}

Evaluating translation quality remains an ongoing challenge in MT research. Traditional automatic evaluation metrics such as BLEU, CHR-F, and METEOR have been widely used, but they often fail to capture semantic correctness and fluency in LLM-generated translations~\cite{baek2023towards}. Recent studies indicate that LLMs themselves can function as robust translation quality evaluators, surpassing traditional evaluation metrics in terms of human correlation assessments~\cite{kocmi2023large}. Furthermore, LLMs have demonstrated their ability to conduct zero-shot and reference-free translation quality estimation, reducing reliance on costly human-labeled evaluation datasets~\cite{huang2023towards}.

\subsection{Research Objectives}

This study aims to compare the performance of LLM-based translation systems and traditional MT models in translating medical documents, focusing on Arabic, Simplified Chinese, and Vietnamese, which are among the most spoken languages other than English in Australia~\cite{language}. The study will evaluate translation quality across multiple dimensions, including linguistic accuracy, terminology retention, discourse coherence, and fluency, using both automatic metrics and human assessment techniques. By investigating the comparative performance of LLM-based and traditional MT systems in medical translation, this research seeks to identify the key strengths and limitations of each approach, contributing to the broader discussion of LLM viability in domain-specific translation tasks.


==> sections/res_backup.tex <==
\section{Results}
\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figs/LLMres.png}
    \caption{Performance comparison of different LLMs and MTs on translating palliative care summaries using automatic metrics. \textcolor{red}{a)......; b)......; c)......
    }}
    \label{fig:enter-label}
\end{figure*}

\subsection{Simple vs. Complex}

\textcolor{red}{Fig. \ref{fig:enter-label} presents a comparative analysis of the three LLMs and the three traditional MT tools on the medical conversation translation task, regarding their performance on BLEU, CHR-F, and METEOR. Fig. 1(a)......; Fig. 1(b)......; Fig. 1(c)......; Fig. 1(d)......; Fig. 1(e)......; Fig. 1(f).......}
Simple summaries, which contain high-level health information and general patient recommendations, yielded consistently higher BLEU scores across all models.
This suggests that both LLMs and traditional MT systems effectively translate general medical content, likely due to their extensive exposure to common health-related terminology in training datasets.
Traditional MT models, including Microsoft Translator (MS) and Google Translate (GTrans), demonstrated strong performance in this category, likely benefiting from large-scale parallel corpora optimized for general language translation.

In contrast, complex summaries, which include specific medical terminology, such as medication names, symptoms, and diagnoses, presented greater challenges to translation models.
The BLEU and CHR-F \textcolor{red}{(METEOR?)} scores dropped significantly for Simplified Chinese and somewhat for Vietnamese, suggesting that existing models struggle with accurately translating technical medical terminology in both languages.
Furthermore, the METEOR scores were lower for complex summary, indicating that the semantic accuracy of the translations was adversely affected by increased linguistic and domain-specific complexity.

However, we observe that the complex summary yields a higher score than the simple one \textcolor{red}{for Arabic}. 
This may be because Arabic is a morphologically rich language, where words undergo complex inflectional changes based on tense, gender, number, and case.
This linguistic feature presents challenges for machine translation models, particularly when translating shorter texts such as the simple summary.
In a shorter context, there are fewer contextual clues for the model to accurately determine the correct morphological form of a word, increasing the risk of mistranslations.
In contrast, the complex summary, which contains more context and a greater density of domain-specific terminology, offers additional linguistic markers that aid in disambiguating words and phrases.
Consequently, models may perform better on longer, more complex texts, where grammatical relationships are more apparent, leading to higher translation quality scores for Arabic in comparison to simpler, less structured summaries.

\subsection{LLMs vs. Traditional MT}
The experimental results indicate that traditional machine translation (MT) models outperform large language models (LLMs) according to established automatic evaluation metrics such as BLEU, CHR-F, and METEOR.
We posit that this performance gap may be attributable, at least in part, to the inherent design of these metrics and the systems they evaluate.
Traditional MT systems are typically optimized to maximize scores on these metrics, which predominantly focus on sentence-level fidelity and lexical overlap with reference translations.
In contrast, LLMs often generate translations that consider broader contextual coherence, discourse-level consistency, and improved readability at the document level.
As a result, LLM-generated translations may involve paraphrasing or restructuring content to improve fluency and cohesion, which, although beneficial from the perspective of a human reader, can be penalized by automatic metrics as they prioritize surface-level similarity over deeper semantic or pragmatic equivalence.

\subsection{Language-Specific Performance Trends}
Across languages, Arabic and Vietnamese exhibited more stable translation performance between simple and complex summaries.
This suggests that medical terminology in these languages is more effectively covered within the training data of both the LLM and MT systems.
In contrast, simplified Chinese translations showed the most significant performance decline in complex summaries, particularly in BLEU scores.
This disparity may be attributed to the linguistic challenges of handling transliterated medical terms, complex syntactic structures, and domain-specific terminology, which are often inconsistently represented in Chinese-language corpora.
